Syll: Open-Source Personal Automation with Cross-Surface Execution

Personal AI agents must increasingly operate across APIs, shells, web surfaces, and desktop GUIs, yet many systems remain tuned to a single interface and offer limited support for user teaching and auditability. We present Syll, an open-source, self-hosted multimodal agent harness that unifies MCP/API tools, CLI execution, and visual GUI control in a modular runtime, enabling agents to coordinate computer use across heterogeneous interfaces while streamlining how users and agents exchange information. At the core of Syll is a bidirectional user-agent interaction layer: users teach procedures through direct demonstration, which Syll compiles into reusable skills; agent execution is translated back into multimodal evidence -- logs, keyframes, and approval checkpoints -- for inspection and control. Syll further externalizes memory, skills, routines, and governance as editable local artifacts, supporting straightforward inspection, extension, and downstream development. Our implementation has been validated on production desktop applications including Adobe Photoshop, Adobe Audition, Stardew Valley, macOS Finder and others. We report mechanism-oriented studies that validate multimodal routing, teachable GUI replay, and persistent local artifacts. We hope Syll can serve as a practical open-source foundation for personal automation that users can teach, inspect, and continuously extend.

==> figures/agent-loop-triangle.tex <==
\begin{tikzpicture}[
  font=\small,
  card/.style={rounded corners=8pt, draw=ivgblue!65!black, line width=0.9pt, fill=ivgblue!6, align=center},
  centerbox/.style={rounded corners=14pt, draw=black!55, line width=1pt, fill=black!4, align=center},
  arr/.style={-{Latex[length=3mm]}, line width=1.1pt, color=ivgblue!80!black},
  keyword/.style={font=\footnotesize, text=black!78}
]
  \coordinate (A) at (0,2.35);
  \coordinate (B) at (-3.0,-1.95);
  \coordinate (C) at (3.0,-1.95);

  \fill[ivgblue!4] (A) -- (B) -- (C) -- cycle;
  \draw[ivgblue!40, line width=0.8pt] (A) -- (B) -- (C) -- cycle;

  \node[card, minimum width=3.6cm, minimum height=1.75cm] (problem) at (A)
    {\textbf{Problem Formulation}\\[1mm]
    {\footnotesize task decomposition}\\
    {\footnotesize interface mismatch}\\
    {\footnotesize human bottleneck}};

  \node[card, minimum width=3.65cm, minimum height=1.75cm] (design) at (B)
    {\textbf{Technical Design}\\[1mm]
    {\footnotesize multimodal control}\\
    {\footnotesize teachability}\\
    {\footnotesize modular runtime}};

  \node[card, minimum width=3.85cm, minimum height=1.75cm] (verify) at (C)
    {\textbf{Runtime Verification}\\[1mm]
    {\footnotesize auditability}\\
    {\footnotesize evidence checkpoints}\\
    {\footnotesize human-in-the-loop}};

  \node[centerbox, minimum width=2.8cm, minimum height=1.2cm] (center) at (0,-0.1)
    {\textbf{Agent Harness}\\[-0.2mm]\footnotesize intent $\leftrightarrow$ action $\leftrightarrow$ evidence};

  \draw[arr] ($(problem.south west)+(0.35,-0.12)$) .. controls (-2.15,0.2) and (-2.55,-0.75) .. ($(design.north east)+(0.05,0.22)$);
  \draw[arr] ($(design.east)+(0.2,0.05)$) .. controls (0.05,-2.85) and (2.0,-2.75) .. ($(verify.west)+(-0.2,0.05)$);
  \draw[arr] ($(verify.north west)+(-0.02,0.22)$) .. controls (2.65,0.9) and (1.1,2.55) .. ($(problem.south east)+(-0.38,-0.1)$);

  \draw[ivgblue!38, dashed] (center.north) -- ($(problem.south)+(0,-0.12)$);
  \draw[ivgblue!38, dashed] (center.south west) -- ($(design.north east)+(0.12,-0.12)$);
  \draw[ivgblue!38, dashed] (center.south east) -- ($(verify.north west)+(-0.12,-0.12)$);
\end{tikzpicture}


==> figures/complexity-throughput-proxy.tex <==
\begin{tikzpicture}[
  x=1cm,y=1cm,
  font=\small,
  axis/.style={line width=0.9pt, -{Latex[length=2.6mm]}, color=black!75},
  grid/.style={color=black!12, line width=0.5pt},
  ailine/.style={color=ivgblue!85!black, line width=1.4pt},
  humanline/.style={color=orange!80!black, line width=1.2pt},
  ptai/.style={circle, fill=ivgblue!85!black, inner sep=1.6pt},
  pthuman/.style={circle, fill=orange!80!black, inner sep=1.4pt},
  ann/.style={font=\footnotesize, align=left, text=black!80}
]
  \def\xmin{0.8}
  \def\xmax{9.9}
  \def\ymin{0.7}
  \def\ymax{6.2}

  \foreach \y in {1.5,2.5,3.5,4.5,5.5} {
    \draw[grid] (\xmin,\y) -- (\xmax,\y);
  }
  \foreach \x/\lbl in {1.2/2023,3.0/2024,4.8/2025,6.6/2026,8.4/2027} {
    \draw[grid] (\x,\ymin) -- (\x,\ymax);
    \node[font=\footnotesize] at (\x,0.42) {\lbl};
  }

  \draw[axis] (\xmin,\ymin) -- (\xmax,\ymin);
  \draw[axis] (\xmin,\ymin) -- (\xmin,\ymax);

  \node[font=\footnotesize] at (5.35,0.05) {Year};
  \node[font=\footnotesize, rotate=90] at (0.02,3.55) {Effective task-complexity throughput (proxy)};

  % Human line
  \draw[humanline] (1.15,1.45) .. controls (2.9,1.58) and (4.9,1.72) .. (6.7,1.88)
                   .. controls (7.7,1.96) and (8.55,2.05) .. (9.15,2.12);
  \node[pthuman] at (1.15,1.45) {};
  \node[pthuman] at (4.8,1.72) {};
  \node[pthuman] at (6.7,1.88) {};
  \node[pthuman] at (9.15,2.12) {};
  \node[ann, anchor=west, text width=2.65cm] at (7.25,2.45)
    {\textbf{Human QA / review bandwidth}\\slow growth, bounded by time and attention};

  % AI line
  \draw[ailine] (1.15,1.08) .. controls (2.15,1.22) and (2.55,1.48) .. (3.0,1.9)
                .. controls (3.7,2.45) and (4.2,2.95) .. (4.8,3.45)
                .. controls (5.45,4.12) and (6.0,4.82) .. (6.6,5.45)
                .. controls (7.15,5.82) and (8.15,6.02) .. (9.1,6.05);
  \node[ptai] at (1.15,1.08) {};
  \node[ptai] at (3.0,1.9) {};
  \node[ptai] at (4.8,3.45) {};
  \node[ptai] at (6.6,5.45) {};
  \node[ptai] at (9.1,6.05) {};

  \node[ann, anchor=west, text width=2.55cm] at (6.05,5.8)
    {\textbf{Agent-side capability / throughput}\\rapid gains from benchmarked agents and high-throughput engineering loops};

  \node[ann, anchor=west, text width=2.15cm] at (3.22,2.18)
    {WebArena / SWE-bench era};
  \node[ann, anchor=west, text width=2.35cm] at (5.02,3.72)
    {OSWorld + computer-use agents};
  \node[ann, anchor=west, text width=2.55cm] at (6.85,4.9)
    {2026 harness-engineering throughput jump};

  \draw[dashed, color=black!35] (6.6,\ymin) -- (6.6,5.5);
  \node[ann, anchor=south west, text width=2.65cm] at (6.72,1.0)
    {Interpretive inflection: generated action rises faster than review capacity.};

  \node[ann, anchor=north west, text width=8.6cm] at (1.0,6.05)
    {Anchors: SWE-bench (software issues), WebArena (web tasks), OSWorld (computer use), and OpenAI's 2026 harness-engineering report. Proxy chart for argumentation, not a direct physical measurement.};
\end{tikzpicture}


==> figures/interface-pyramid.tex <==
\begin{tikzpicture}[
  font=\small,
  layer/.style={draw=ivgblue!70, fill=ivgblue!7, rounded corners=2pt, minimum height=0.65cm, align=center},
  loopbox/.style={draw=black!45, fill=black!3, rounded corners=2pt, align=center},
  arr/.style={-{Latex[length=2.2mm]}, thick, black!65},
  note/.style={align=center, font=\footnotesize}
]
  \node[layer, minimum width=6.6cm] (gui) at (0,0) {GUI / visual surface\\human-visible state, screenshots, mouse and keyboard};
  \node[layer, minimum width=5.1cm] (cli) at (0,0.86) {CLI / shell\\deterministic local execution};
  \node[layer, minimum width=3.6cm] (api) at (0,1.72) {MCP / API / tools\\structured machine interfaces};

  \node[draw=ivgblue, rounded corners=4pt, fit=(gui)(cli)(api), inner xsep=0.35cm, inner ysep=0.25cm,
        label={[font=\small\bfseries, text=ivgblue]above:Syll harness}] (harness) {};

  \node[loopbox, minimum width=2.55cm, minimum height=0.62cm, right=1.45cm of cli] (demo) {Demonstration\\capture};
  \node[loopbox, minimum width=2.55cm, minimum height=0.62cm, below=0.45cm of demo] (skills) {Skill library};
  \node[loopbox, minimum width=2.55cm, minimum height=0.62cm, below=0.45cm of skills] (replay) {Replay / schedule};

  \draw[arr] (demo) -- (skills);
  \draw[arr] (skills) -- (replay);
  \draw[arr] (replay.west) to[out=180,in=0] ($(gui.east)+(0,0.03)$);
  \draw[arr] ($(gui.east)+(0,0.13)$) to[out=0,in=180] (demo.west);

  \node[note, below=0.35cm of gui] (memory) {Memory, sessions, channels, and context builder keep the surfaces aligned.};
  \draw[arr] (memory.north) -- ($(gui.south)+(0,-0.02)$);
\end{tikzpicture}


==> figures/syll-framework.tex <==
\begin{tikzpicture}[
  x=1cm,y=1cm,
  font=\small,
  panel/.style={rounded corners=10pt, draw=black!35, line width=0.9pt, fill=black!2},
  box/.style={rounded corners=6pt, draw=ivgblue!70!black, line width=0.8pt, fill=ivgblue!7, align=center},
  warmbox/.style={rounded corners=6pt, draw=orange!70!black, line width=0.8pt, fill=orange!11, align=center},
  softbox/.style={rounded corners=6pt, draw=teal!60!black, line width=0.8pt, fill=teal!10, align=center},
  ghostbox/.style={rounded corners=7pt, draw=black!55, line width=0.8pt, fill=black!5, align=center},
  arr/.style={-{Latex[length=2.6mm]}, line width=0.95pt, color=black!70},
  note/.style={font=\footnotesize, text=black!75, align=center}
]
  % Left panel
  \node[panel, minimum width=4.2cm, minimum height=8.3cm, anchor=north west] (leftpanel) at (0,0) {};
  \node[font=\bfseries] at (2.1,-0.42) {Complementary Work Surfaces};
  \node[note, text width=3.65cm] at (2.1,-0.88) {The same task can descend or climb across interfaces depending on observability and control needs.};

  \node[box, minimum width=2.2cm, minimum height=0.84cm] (mcp) at (2.1,-1.7) {\textbf{MCP / API}\\\footnotesize structured access};
  \node[box, minimum width=2.8cm, minimum height=0.9cm] (cli) at (2.1,-2.8) {\textbf{CLI / Shell}\\\footnotesize deterministic local actions};
  \node[box, minimum width=3.45cm, minimum height=1.05cm] (gui) at (2.1,-4.15) {\textbf{GUI / Visual Surface}\\\footnotesize screenshots, windows, mouse, keyboard};
  \draw[ivgblue!45, line width=0.8pt] ($(mcp.north west)+(-0.25,0.12)$) -- ($(gui.south west)+(-0.25,-0.15)$) -- ($(gui.south east)+(0.25,-0.15)$) -- ($(mcp.north east)+(0.25,0.12)$);

  \node[softbox, minimum width=3.4cm, minimum height=0.92cm] (teach) at (2.1,-5.7) {\textbf{Demonstration Input}\\\footnotesize record once, annotate once};
  \node[softbox, minimum width=3.4cm, minimum height=0.92cm] (audit) at (2.1,-7.0) {\textbf{Evidence Output}\\\footnotesize previews, screenshots, attachments};
  \draw[arr] (teach) -- (audit);

  % Center panel
  \node[panel, minimum width=6.9cm, minimum height=8.3cm, anchor=north west] (midpanel) at (4.6,0) {};
  \node[font=\bfseries] at (8.05,-0.42) {Syll Runtime Core};

  \node[box, minimum width=2.1cm, minimum height=0.9cm] (channels) at (5.85,-1.35) {\textbf{Channels / UI}\\\footnotesize web, CLI, chat};
  \node[box, minimum width=2.2cm, minimum height=0.9cm] (context) at (8.15,-1.35) {\textbf{Context Builder}\\\footnotesize prompt + media assembly};
  \node[box, minimum width=2.1cm, minimum height=0.9cm] (memory) at (10.2,-1.35) {\textbf{Memory}\\\footnotesize notes, identity, fragments};

  \node[warmbox, minimum width=2.05cm, minimum height=0.9cm] (skills) at (5.8,-3.0) {\textbf{Skill Library}\\\footnotesize markdown + recorded};
  \node[warmbox, minimum width=2.25cm, minimum height=0.9cm] (recorder) at (8.15,-3.0) {\textbf{Recorder / Convertor}\\\footnotesize demo $\rightarrow$ workflow};
  \node[warmbox, minimum width=2.0cm, minimum height=0.9cm] (sessions) at (10.25,-3.0) {\textbf{Sessions}\\\footnotesize history, routing};

  \node[ghostbox, minimum width=2.55cm, minimum height=1.0cm] (loop) at (6.3,-5.0) {\textbf{Planner--Agent Loop}\\\footnotesize infer, call, reflect};
  \node[ghostbox, minimum width=2.55cm, minimum height=1.0cm] (tools) at (9.6,-5.0) {\textbf{Tool Registry}\\\footnotesize files, shell, web, GUI};
  \node[ghostbox, minimum width=4.95cm, minimum height=0.95cm] (verify) at (7.95,-6.8) {\textbf{Verification Path}\\\footnotesize checkpoints, previews, screenshots, monitor alerts};

  \draw[arr] (channels) -- (context);
  \draw[arr] (memory) -- (context);
  \draw[arr] (skills) -- (context);
  \draw[arr] (recorder) -- (skills);
  \draw[arr] (sessions) -- (context);
  \draw[arr] (context) -- (loop);
  \draw[arr] (loop) -- (tools);
  \draw[arr] (tools) -- ++(0,0.95) -| (context.south);
  \draw[arr] (tools) -- (verify);
  \draw[arr] (verify.west) -- ++(-1.45,0) |- (channels.south);

  % Right panel
  \node[panel, minimum width=4.9cm, minimum height=8.3cm, anchor=north west] (rightpanel) at (12.1,0) {};
  \node[font=\bfseries] at (14.55,-0.42) {Representative Tasks};

  \node[ghostbox, minimum width=3.8cm, minimum height=1.0cm] (task1) at (14.55,-1.45) {\textbf{Recorded Workflow Replay}\\\footnotesize execute a taught browser or desktop routine};
  \node[ghostbox, minimum width=3.8cm, minimum height=1.0cm] (task2) at (14.55,-2.95) {\textbf{Scheduled Ritual / Briefing}\\\footnotesize proactive check-ins with optional silence};
  \node[ghostbox, minimum width=3.8cm, minimum height=1.0cm] (task3) at (14.55,-4.45) {\textbf{Phone-to-Desktop Retrieval}\\\footnotesize locate, preview, confirm, and return files};
  \node[ghostbox, minimum width=3.8cm, minimum height=1.0cm] (task4) at (14.55,-5.95) {\textbf{Cross-App GUI Automation}\\\footnotesize act across apps when no robust API exists};

  \draw[arr] (tools.east) -- ++(0.85,0) |- (task1.west);
  \draw[arr] (verify.east) -- ++(1.15,0) |- (task2.west);
  \draw[arr] (channels.east) -- ++(5.15,0) |- (task3.west);
  \draw[arr] (loop.east) -- ++(4.15,0) |- (task4.west);

  % Subtle Syll visual cue
  \begin{scope}[shift={(14.5,-7.45)}]
    \fill[black!82] (0,0) ellipse (0.63 and 0.12);
    \fill[white] (0,0.38) .. controls (-0.42,0.38) and (-0.5,-0.2) .. (-0.42,-0.48)
                  .. controls (-0.27,-0.88) and (0.27,-0.88) .. (0.42,-0.48)
                  .. controls (0.5,-0.2) and (0.42,0.38) .. (0,0.38) -- cycle;
    \fill[black!85] (-0.12,0.18) ellipse (0.045 and 0.09);
    \fill[black!85] (0.12,0.18) ellipse (0.045 and 0.09);
    \draw[black!70, line width=0.7pt] (-0.35,-0.12) -- (0.35,-0.12);
    \fill[black!90] (-0.37,-0.12) -- (0.25,-0.12) -- (0.43,-0.34) -- (-0.18,-0.34) -- cycle;
  \end{scope}

  \node[note, text width=4.05cm] at (14.55,-8.0) {A small visual cue echoes the Syll identity while keeping the figure schematic and paper-friendly.};
\end{tikzpicture}

